Circular-Symmetric Correlation Layer based on FFT

Despite the vast success of standard planar convolutional neural networks, they are not the most efficient choice for analyzing signals that lie on an arbitrarily curved manifold, such as a cylinder. The problem arises when one performs a planar projection of these signals and inevitably causes them to be distorted or broken where there is valuable information. We propose a Circular-symmetric Correlation Layer (CCL) based on the formalism of roto-translation equivariant correlation on the continuous group $S^1 \times \mathbb{R}$, and implement it efficiently using the well-known Fast Fourier Transform (FFT) algorithm. We showcase the performance analysis of a general network equipped with CCL on various recognition and classification tasks and datasets. The PyTorch package implementation of CCL is provided online.

==> Checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In figure.~\ref{fig:acc}(c) and (d)}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{In section.~3.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{In section.~3.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{in the supplemental material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Randomized results for accuracy is obtained in section.~4}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{in the supplemental material}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In Section.~2 and section.~4.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{In supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> TEX/Extra.tex <==


\paragraph{\cite{maron2020learning}}
less emphasis has been
given to the common case where set elements
themselves adhere to their own symmetries.

That
case is relevant to numerous applications, from
deblurring image bursts to multi-view 3D shape
recognition and reconstruction.

In this setting, each data point consists of a set of elements,
and the task is independent of element order. This independence
induces a symmetry structure, which can be used
to design deep models with improved efficiency and generalization.

However, in many
cases, the elements of the set themselves adhere to certain
symmetries, as happens when learning with sets of images,


However, in many
cases, the elements of the set themselves adhere to certain
symmetries, as happens when learning with sets of images,
sets of point-clouds and sets of graphs.


A common approach to handle per-element symmetries, is
based on processing elements individually.



First, we describe the symmetry
group of these sets, and then fully characterize the
space of linear layers that are equivariant to this group. Notably,
this characterization implies that information between
set elements should be shared in all layers.

A potential concern with equivariant architectures is that
restricting layers to be equivariant to some group of symmetries
may reduce the expressive power of the model (Maron
et al., 2019c; Morris et al., 2018; Xu et al., 2019).




\section{Previous work}
\paragraph{[Ravan] Equivariance through parameter-sharing}
\begin{itemize}
    \item $G$-equivariance under some conditions on the actions of $G$.
    \item sensitivity to all other permutation groups outside $G$. 
    \item \textbf{What kind of priors on input/output structure can be encoded through parameter-sharing?} This work is an attempt at answering this question, when our priors are in the form discrete domain symmetries. To formalize this type of prior, a family of transformations of input and output to a neural layer are expressed as group “action” on the input and output.
    \item \textbf{Parameter-sharing}: simplicity and computational efficiency.
    \item \textbf{steerable filters}:
    
    \item Due to the discrete nature of parameter-sharing, our treatment here is limited to permutation groups. Action of a permutation group $G$ can model discrete transformations of a set of variables, such as translation and $90^{\circ}$  rotation of pixels around any center in an image.
    \item The core idea is simple: consider a colored bipartite graph representing a neural network layer. Edges of the same color represent tied parameters. This neural network layer as a function is equivariant to the actions of a given group $\mathcal{G}$ (and nothing more) iff the action of $\mathcal{G}$ is the symmetry group of – i.e., there is a simple bijection between parameter symmetries and equivariences of the corresponding neural network.
    
    \item $\vec{\mathbb{N}}$ is ordered counterpart of $\mathbb{N}$.
    \item  
\end{itemize}
\paragraph{[Cohen] Gauge Equivariant CNN}
\begin{itemize}
    \item General principle to guide architecture search.
    \item One such rational design principle maintains that maintains that
network architectures should be equivariant to symmetries.
    \item However, manifolds do not in general have global symmetries, and so it is not obvious how one might develop equivariant CNNs for them.
    \item we define a convolution-like operation on general manifolds $M$ that is equivariant to local gauge transformations.
    \item Each field is represented by a number of feature maps, whose activations are interpreted as the coefficients of a geometrical object (e.g. scalar, vector, tensor, etc.) relative to a spatially varying frame (i.e. gauge).
    \item Segmentation of omnidirectional signal.
    \item Results on IcoMNIST, climate pattern segmentation, and omnidirectional RGB-D image segmentation
    \item We define a gauge as a position-dependent invertible linear map $w_p : \mathbb{R}^d \rightarrow T_pM$, where $T_pM$ is the tangent space of $M$ at $p$. This determines a frame $w_p(e_1), \dots, w_p(e_d)$ in $T_pM$, where $\{e_i\}$ is the standard frame of $\mathbb{R}^d$.
    \item  
    
    
    
    
\end{itemize}


\paragraph{[Bartok] Models of active learning in group-structured state spaces}




\paragraph{\cite{wang2021incorporating}:}Research into equivariant neural networks has mostly been applied to tasks such as image classification
and segmentation [27; 50; 49]. In contrast, we design equivariant networks in a completely different
context, that of a time series representing a physical process.

but since the symmetries we focus on are pervasive in almost all physics problems, we expect our techniques will be widely applicable. Our contributions include:

*We design tailored methods with theoretical guarantees to incorporate various symmetries, including
uniform motion, rotation, and scaling, into convolutional neural networks.

*When evaluated on turbulent convection and ocean current prediction, our models achieve significant
improvement on generalization of both predictions and physical consistency.

*Parameters: For different symmetries, our methods have an average 31\% and maximum 78\% reduction in energy error when evaluated on turbulent convection with no distributional shift.


\paragraph{What is important in considering equivariance of the network architecture with respect to the action of a given group $G$}
\begin{itemize}
    \item $G$-equivariance is not restrictive enough a family
    \item there is the issue of the network expressivity
    \item in other words, the function 
\end{itemize}

==> TEX/algo.tex <==

%\algg
\newcommand{\algg}{
\begin{algorithm}[H]
\caption{\texttt{CCL} class}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\SetKwInput{KwInit}{Initialize} 
\DontPrintSemicolon


  %\KwData{Testing set $x$}
% Set Function Names
  \SetKwFunction{FMain}{Main}
  \SetKwFunction{FSum}{CCL}
  \SetKwFunction{FSub}{Forward}

% Write Function with word ``Function''
  \SetKwProg{Fn}{Class}{:}{}
  \Fn{\FSum{$C_\textsc{in}$, $C_\textsc{out}$, $k_h$, $k_w$, $s_h$, $s_w$}}{ 
        \;
        \textbf{Parameters:} 
        $W_{\textsc{fft}}\in \mathbb{R}^{C_\textsc{out}\times C_\textsc{in} \times k_w}$, $W_{\textsc{dct}}\in \mathbb{R}^{C_\textsc{out}\times C_\textsc{in} \times k_h}$, $b\in \mathbb{R}^{C_\textsc{out}}$\;
        \;
        
          \KwInput{$X \in \mathbb{R}^{C_\textsc{in}\times H \times W}$}
  \KwOutput{$F \in \mathbb{R}^{C_\textsc{out}\times \ceil*{\frac{H}{s_h}} \times \ceil*{\frac{W}{s_w}}}$}
  \;
        
% Write Function with word ``Def''
  \SetKwProg{Fn}{Def}{:}{}
  \Fn{\FSub{X}}{
        $F\leftarrow \texttt{DCT}_{\textsc{h}}(X)\odot\texttt{DCT}(W_{\textsc{dct}})$\;
        $F\leftarrow \texttt{DCT}^{-1}_{\textsc{h}}(F)$\;
        $F\leftarrow \texttt{FFT}_{\textsc{w}}(F)\odot\texttt{FFT}(W_{\textsc{fft}})$\;
        $F\leftarrow \mathlarger{\sum}_{C_\textsc{in}} F$\;
        $F\leftarrow \texttt{FFT}^{-1}_{\textsc{w}}(F)$\;
        \KwRet $\texttt{subsample}(F, s_h, s_w)$\;
  }
  \;
        
  }
\end{algorithm}
}



==> TEX/keywords.tex <==

group $\mathbb{z}$
subgroup $5\mathbb{z}$
normal subgroup $5\mathbb{z}$
coset
quotient group $\mathbb{z}\mathbin{/}5\mathbb{z}$
quotient group is not a subgroup of $\mathbb{z}$
cannot call it a subgroup if the cosets do not form a group.
Faithful
direct product
simple group, factor group (abstract algebra)
